Enclosed Loops: How open source communities become datasets

Centralization in code hosting and package management in the 2010s created fundamental shifts in the social arrangements of open source ecosystems. In a regime of centralized open source, platform effects can both empower and detract from communities depending on underlying technical implementations and governance mechanisms. In this paper we examine Dependabot, Crater and Copilot as three nascent tools whose existence is predicated on centralized software at scale. Open source ecosystems are maintained by positive feedback loops between community members and their outputs. This mechanism is guided by community standards that foreground notions of accountability and transparency. On one hand, software at scale supports positive feedback loops of exchange among ecosystem stakeholders: community members (developers), users, and projects. On the other, software at scale becomes a commodity to be leveraged and expropriated. We perform a comparative analysis of attributes across the three tools and evaluate their goals, values, and norms. We investigate these feedback loops and their sociotechnical effects on open source communities. We demonstrate how the values embedded in each case study may diverge from the foundational ethos of open communities as they are motivated by, and respond to the platform effects, corporate capture, and centralization of open source infrastructure. Our analysis finds that these tools embed values that are reflective of different modes of development - some are transparent and accountable, and others are not. In doing so, certain tools may have feedback mechanisms that extend communities. Others threaten and damage communities ability to reproduce themselves.

==> 02_RelatedWork.tex <==
\section{Related Work}

 The development and growth of open source ecosystems relied on innovations in licensing that have created complex edge case around what constitutes free use in both the legal and ethical sense \cite{grimmelmann2015copyright}. In their work, \citet{EthicsAIOpenSource} argue for greater scrutiny of the ethical deployment of Open Source AI projects, and the resulting ``downstream harms'' they might cause which are insufficiently mitigated under current norms or legal practices \cite{cooper2023variance}.
\citet{CounterFAccTual} argue that by just focusing on fairness in AI-oriented projects solely at the ``design" phase, we are risking missing issues in deployment contexts. However, in many cases, the downstream control assumption is challenging to perform because of large data and computational resource requirements. To address these issues, \citet{BehavioralUseLicensing} examined licensing approaches based on Apache 2.0 to help with  downstream control of open-source  large-scale trained AI models that cannot be easily replicated in an academic setting.

We highlight prior works on examination of ethical issues of open-source AI projects and governance structure needed to encourage voluntary community members participation and quality contributions.
\citet{Linar2022} find that designing governance around participation and contributions rather than close monitoring and sanctions would ``[promote] sustainability of open data and the potential value it can provide in existing and future ecosystems''. Open source ecosystems are, by their nature required to create mechanisms that allow them to continuously reproduce and grow their communities. Communities are at risk of ``Underproduction'' in digital infrastructures that depend on voluntary maintenance contributions \cite{SociotechnicalRisk,9426043,curto2022sustainability}.

% Drawing on the FAccT community scholarship on accountability, transparency, and ethical considerations in building information systems, 
Our work explores how open-source communities software outputs were transformed into novel datasets whose uses may or may not conform with the vision, values, and norms of those communities

% that predicated the development of software operating on large-scale source repositories. Specifically, what shaped the communities' institutions and whether the systems that were built on in those communities share their vision, values, and norms.



% As a possible alternative, \citet{TechWorkerOrganiz} argue that tech-workers behind the product can serve de facto guardians ``against strong corporate impulses to grow or make a profit to the detriment of other values. The work examines successful collective campaigns ' and looks at existing publications on worker organizing\cite{mcalevey2015no} on US labor movements \cite{mcalevey2015no}. Building on \citet{sharp1973politics}'s  framework of nonviolent actions, the authors propose a refined framework to help workers organize to induce effective change. 


%Software contributions and usage face a similar issues where digital infrastructure depends on the voluntary maintenance contributions~\cite{SociotechnicalRisk}, we run the risk of what~\citet{9426043} call ``Underproduction''\cite{9426043}.


%\chcomment{YS: My attempt at a summary paragraph. Somebody should go over it for sanity check and possible additions.}


%Other efforts attempt to directly bridge the gap between Tech-workers and those affected by the policy through workshop sessions, as shown by 
%\citet{CreatingCommunityBasedTechPolicy}.
%\subsection{Reaching the Community}
%In an attempt to While attention to the design process is essential, other work directly focuses on the impacted communities. \citet{CreatingCommunityBasedTechPolicy} address this issue by directly including communities and their affected members in the design process. In their workshop, they attempted to bridge the gap between AI practitioners and marginalized communities impacted by the implemented communities.  

%\citet{DisclosurebyDesign} address the problem of the community by defining a technical disclosure interface with the goal of ``...supporting effective transparency and oversight.'' and to have the public be ``...meaningfully inform[ed]'' as they get impact by decisions made from an AI. 



%Using software at scale? While The advancements in Large Language models are very recent \cite{gpt3}, the idea to use open-source code as training material is not. Some early work on this goes back to 2004\footnote{\url{http://2004.msrconf.org}} \cite{kalliamvakou2016depth}. 



%\citet{EthicsAIOpenSource}  argue that methods to achieve ``Ethical AI'' are often discussed within the FAccT community, aimed at private enterprises developing and deploying AI systems. The authors question to what extent such methods do not (necessarily) carry over to Open Source projects. Not only are other methods necessary, but also an understanding of responsibility by the contributors to the open-source project. The term ``Downstream Control Assumption''~\cite{EthicsAIOpenSource} is introduced to characterize how an entity, public or private, reasons about its control of a project after its publication.


%The lack of consideration downstream Control has also been identified in other FAccT submissions. \citet{CounterFAccTual} argue that many submissions that strive to supply provide methods to ensure fairness in AI-oriented projects only address issues during the early "design" phase and are often missing implementation contexts.  



%Other work has looked at how a specific licensing approach could help with the downstream control of open-source and academic work\cite{BehavioralUseLicensing}. \citet{BehavioralUseLicensing} further extends this argument to include large-scale and trained AI models (e.g. OpenAI's GPT-3) where both the data and computational resources used fall outside of what can be replicated easily. The authors present an example license based on Apache 2.0 as a starting point. 


%Other attempts to ensure the Ethical Use of AI  have looked at the tech worker community and argued it as a Collective Action task \cite{TechWorkerOrganiz}. \citet{TechWorkerOrganiz} looked at existing publications on worker organizing, in particular, work by \citet{mcalevey2015no} on US labor movements \cite{mcalevey2015no} as well as work by Sharp\cite{sharp1973politics}.

%The objective is to balance ``...transparency, proprietorship, privacy, and research objectives.'' \cite{BeyondOpencsClosed} remains the same and a conundrum for the FAccT Community.  \citet{BeyondOpencsClosed} addresses this gap by providing: ``synthetic datasets that offer a) strong privacy guarantees, b) removal of signals that could expose competitive advantage, and c) removal of biases that could reinforce discriminatory policies, all while maintaining fidelity to the original data.''




%\begin{itemize}
%\item https://dl.acm.org/doi/10.1145/3531146.3533137
%\end{itemize}



%``Montr\'eal Declaration for a Responsible Development of Artificial Intelligence'' \cite{} cannot address.






%\subsection{How to consider conflicts of interest within FAcct}


% \subsection{Impact of tools on code and communities} / not Faact
% Research on understanding how different software development tools impact communities and software has been a long-standing research effort within the Software Engineering field.

%   * Centralized version control vs. Decentralized version control (  a historical note) \cite{10.1145/2568225.2568322} Using decentralized systems such as Git benefits the code that gets produced.
% -software engineering community 

% \cite{8778723} Many developers use version control systems (GitHub) to look for information and prepare their work to be used as a source of information.  However, the infrastructure on which decentralized version control algorithms are running has experienced a form of centralization. 



%While there has been significant analysis of AI/ML-based systems and their designs, we could also highlight how factors around predominantly open-source development play a role in how risk(maintenance), use( vision and Downstream control) and ,values (privacy and quality of data) and norms(governance) need to be evaluated. 

%we demonstrate that the systems can also be placed in a broader context of software systems that use existing code as a material resource.


%Prior work on open-source software development and communities have heavily focus ---- . Related work can be organized into X categories: work that focuses on (1) methods to address fairness (2) norms (3) copyright and legal issues, (4) ---- and so on.



%\subsection {Downstream Harms}
%\chadded[id=YS, comment=my version of the below text. Feel free to use or delete.]{

